Strategy Synthesis for Surveillance-Evasion Games with Learning-Enabled Visibility Optimization

This paper studies a two-player game with a quantitative surveillance requirement on an adversarial target moving in a discrete state space and a secondary objective to maximize short-term visibility of the environment. We impose the surveillance requirement as a temporal logic constraint.We then use a greedy approach to determine vantage points that optimize a notion of information gain, namely, the number of newly-seen states. By using a convolutional neural network trained on a class of environments, we can efficiently approximate the information gain at each potential vantage point.Subsequent vantage points are chosen such that moving to that location will not jeopardize the surveillance requirement, regardless of any future action chosen by the target. Our method combines guarantees of correctness from formal methods with the scalability of machine learning to provide an efficient approach for surveillance-constrained visibility optimization.

==> casestudy.tex <==
\section{Case Study} %{Motivating Example}
We first describe the problem informally, in the context of a motivating case study. Figure~\ref{fig:casestudy} represents an example environment that we represent as a gridworld.

\begin{figure}[h!]
\centering
\subfloat[Surveillance arena \label{fig:map}]{
\includegraphics[width=0.45\linewidth]{figs/unnamed.png}
}
%\hfill
\subfloat[Gridworld representation\label{fig:gridofmap}]{
\includegraphics[width=0.45\linewidth]{figs/gridworldfig_exploration_permissive_32_hq.png}
}
\caption{Sample environment and corresponding gridworld representation. The blue circle corresponds to the controlled agent and the orange circle corresponds to the hostile target. Red cells are obstacles that obscure vision. Black cells in (b) correspond to occlusions.}\label{fig:casestudy}
\end{figure}

We are interested in \emph{patrolling the environment}, i.e., observing all the states in the environment infinitely often given the vision capabilities of the agent. In this example, the agent's observations correspond to line-of-sight sensor measurements, where the sensor range is larger than the domain of interest, as illustrated in Figure~\ref{fig:gridofmap}. Additionally, we require the pursuer (blue) to satisfy a \emph{surveillance requirement} on the target (orange). Informally we specify surveillance requirements in the following way - \emph{always know the location of the target up to some given precision}. We make concrete this notion in the following section. 

We treat the target's actions as non-deterministic - we know what it \emph{can} do, but we have no model for its behaviour. Hence, if we are required to satisfy the surveillance requirement, we cannot guarantee the entire environment can be patrolled. We relax the patrol requirement to \emph{maximizing} the number of states that are visible subject to the surveillance specification. In short, we require a \emph{strategy}, i.e, given the current joint state of the pursuer and target, choose next action of the pursuer that is \emph{correct} with respect to the surveillance requirement but also maximizes visibility of the unseen parts of the map. 

==> figs/simple-abstr-transitions.tex <==
\begin{center}
\vspace{0.2cm}
\begin{tikzpicture}[node distance=.9 cm,auto,>=latex',line join=bevel,transform shape,scale=.8]
\node at (0,0) (s0) {$(4,18)$};
\node  [below left of=s0,yshift=-.2cm,xshift=-.35cm] (s2) {$(3,19)$};
\node  [below right of=s0,yshift=-.2cm,xshift=.35cm] (s3) {$(9,\{Q_4,Q_5\})$};
\node  [left of=s2,xshift=-1cm] (s1) {$(3,\{Q_4,Q_5\})$};
\node  [right of=s3,xshift=1cm] (s4) {$(9,19)$};

\draw [->] (s0) edge (s1.north);
\draw [->] (s0) edge (s2.north);
\draw [->] (s0) edge (s3.north);
\draw [->] (s0) edge (s4.north);
\end{tikzpicture}
\end{center}



==> figs/simple-belief-transitions.tex <==
\begin{center}
\vspace{0.2cm}
\begin{tikzpicture}[node distance=.9 cm,auto,>=latex',line join=bevel,transform shape,scale=.75]
\node at (0,0) (s0) {$(4,\{18\})$};
\node  [below left of=s0,yshift=-.5cm,xshift=-.35cm] (s2) {$(3,\{17,23\})$};
\node  [below right of=s0,yshift=-.5cm,xshift=.35cm] (s3) {$(9,\{19\})$};
\node  [left of=s2,xshift=-1cm] (s1) {$(3,\{19\})$};
\node  [right of=s3,xshift=1cm] (s4) {$(9,\{17,23\})$};

\draw [->] (s0) edge (s1.north);
\draw [->] (s0) edge (s2.north);
\draw [->] (s0) edge (s3.north);
\draw [->] (s0) edge (s4.north);
\end{tikzpicture}
\end{center}


==> figs/simple-safety-counterex-1.tex <==
\begin{tikzpicture}[node distance=.7 cm,auto,>=latex',line join=bevel,transform shape,scale=.75]
\node at (0,0) (s0) {$v_0:(4,18)$};
\node  [below left of=s0,yshift=-.2cm,xshift=-2.2cm] (s1) {$v_1:(3,\{Q_2\})$};
\node  [below right of=s0,yshift=-.2cm,xshift=2.2cm] (s2) {$v_2:(9,\{Q_2\})$};
\node  [below of=s1,yshift=-.2cm] (s4) {$v_4:(4,A)$};
\node  [below of=s2,yshift=-.2cm] (s7) {$v_7:(8,A)$};
\node  [left of=s4,xshift=-1cm] (s3) {$v_3:(2,A)$};
\node  [right of=s4,xshift=1cm] (s5) {$v_5:(8,A)$};
\node  [left of=s7,xshift=-1cm] (s6) {$v_6:(4,A)$};
\node  [right of=s7,xshift=1cm] (s8) {$v_8:(14,A)$};
\draw [->] (s0) edge (s1.north);
\draw [->] (s0) edge (s2.north);
\draw [->] (s1) edge (s3.north);
\draw [->] (s1) edge (s4.north);
\draw [->] (s1) edge (s5.north);
\draw [->] (s2) edge (s6.north);
\draw [->] (s2) edge (s7.north);
\draw [->] (s2) edge (s8.north);

\end{tikzpicture}


==> figs/simple-safety-counterex-abstr.tex <==
\begin{tikzpicture}[node distance=.7 cm,auto,>=latex',line join=bevel,transform shape,scale=.75]
\node at (0,0) (s0) {$(4,18)$};
\node  [below left of=s0,yshift=-.5cm,xshift=-.5cm] (s1) {$(3,\{Q_4,Q_5\})$};
\node  [below right of=s0,yshift=-.5cm,xshift=.5cm] (s2) {$(9,\{Q_4,Q_5\})$};

\draw [->] (s0) edge (s1.north);
\draw [->] (s0) edge (s2.north);
\end{tikzpicture}


==> figs/simple-safety-counterex-concr.tex <==
\begin{tikzpicture}[node distance=.7 cm,auto,>=latex',line join=bevel,transform shape,scale=.75]
\node at (0,0) (s0) {$(4,18)$};
\node  [below left of=s0,yshift=-.5cm,xshift=-.5cm] (s1) {$(3,\{17,23\})$};
\node  [below right of=s0,yshift=-.5cm,xshift=.5cm] (s2) {$(9,\{17,23\})$};

\draw [->] (s0) edge (s1.north);
\draw [->] (s0) edge (s2.north);
\end{tikzpicture}


==> figs/simple-transitions.tex <==
\begin{minipage}{5.0cm}
\vspace{-1.8cm}
{\fontsize{8}{10}\selectfont $\vis(4,18) = \false,\vis(4,17) = \false,$ $\vis(4,19) = \true, \vis(4,23) = \false$}

\smallskip

\begin{tikzpicture}[node distance=.75 cm,auto,>=latex',line join=bevel,transform shape,scale=0.75]
\node at (0,0) (s0) {$(4,18)$};
\node  [below left of=s0,yshift=-.5cm] (s3) {$(3,23)$};
\node  [below right of=s0,yshift=-.5cm] (s4) {$(9,17)$};
\node  [left of=s3,xshift=-.35cm] (s2) {$(3,19)$};
\node  [left of=s2,xshift=-.35cm] (s1) {$(3,17)$};
\node  [right of=s4,xshift=.35cm] (s5) {$(9,19)$};
\node  [right of=s5,xshift=.35cm] (s6) {$(9,23)$};

\draw [->] (s0) edge (s1.north);
\draw [->] (s0) edge (s2.north);
\draw [->] (s0) edge (s3.north);
\draw [->] (s0) edge (s4.north);
\draw [->] (s0) edge (s5.north);
\draw [->] (s0) edge (s6.north);
\end{tikzpicture}
\end{minipage}


==> preliminaries.tex <==
\section{Preliminaries}
\label{sec_prel}



\subsubsection{Two-player Games}
%
A two-player game is a tuple $\game = (\gstates,
\ginit, \alphabet, \delta)$,
where $\gstates$ is a finite set of states, $\ginit \in \gstates$ is the initial state,
$\delta: \gstates \times \alphabet \rightarrow \gstates$
is a complete transition function, $\Acc: (\gstates \times \alphabet \times \gstates)^\omega \rightarrow \bools$ is a winning condition
and defines the qualitative objective of the game.
%
The game is played  by two players:  the system and the environment. In every state $s\in \gstates$
(starting with $\ginit$), the environment chooses an input
$\isymb \in \ialphabet$, and then the system chooses some output $\osymb \in \oalphabet$. These choices define the next state $s' = \delta(s,(\isymb, \osymb))$, and so on. The resulting (infinite)
sequence $\overline{\pi} = (\ginit,\isymb, \osymb, s_1) (s_1,\isymb, \osymb, s_2) \ldots$ is called a \emph{play}.
A deterministic  \emph{strategy} for the environment is a function
$\rho_e: \gstates^* \rightarrow \ialphabet$.
A nondeterministic \emph{strategy} for the system is a relation $\rho_s:
\gstates^* \times \ialphabet \rightarrow 2^{\oalphabet}$ and a
deterministic  strategy for the system is a function $\rho_s:
\gstates^* \times \ialphabet \rightarrow \oalphabet$.\looseness=-1

A play $\overline{\pi}$ is \emph{won} by the system iff $\Acc(\overline{\pi})=\top$.
 A strategy is \emph{winning} for the system if all plays $\overline{\pi}$ that can be
constructed when defining the outputs using the strategy result in
$\Acc(\overline{\pi})=\top$. The \emph{winning region} $\Win$ is the set of states
from which a winning strategy exists.
A \emph{permissive} winning strategy  $\rho_s:
\gstates^* \times \ialphabet \rightarrow 2^{\oalphabet}$ is a strategy that is not only winning for the system, but also contains all deterministic winning strategies.

A \emph{safety game} defines $\Acc$ via a set $F\subseteq \gstates$ of
safe states: $\Acc(\overline{\pi})=\top$ iff $g_i \in F$ for all $i \geq 0$, i.e., if only safe states are visited in the play $\overline{\pi}$. Otherwise, $\Acc(\overline{\pi})=\bot$.
%If a safety game is won by the system player, then there exists a permissive strategy $\rho_s$ that is \emph{memoryless}, i.e., has the form $\rho_s:
%\gstates \times \ialphabet \rightarrow 2^{\oalphabet}$.
%
The \emph{\buchi} winning condition is $\Acc(\overline{\pi})=\top$ iff $\inf(\overline{\pi})
\cap F \neq \emptyset$, where $F \subseteq Q$ is
the set of accepting states and $\inf(\overline{\pi})$ is the set of states that occur infinitely often in $\overline{\pi}$.
We abbreviate the \buchi condition as $\mathcal{B}(F)$.
A \emph{Generalized Reactivity 1} (GR(1))
acceptance condition is a predicate $\bigwedge_{i=1}^{m} \mathcal{B}(E_{i}) \rightarrow \bigwedge_{i=1}^{n} \mathcal{B}(F_{i})$, with
$E_i \subseteq Q$ and $F_i \subseteq Q$.
\looseness=-1
%
\iffalse MEAN-PAYOFF
A \emph{mean-payoff game} is a game where $\Val$ is defined via an edge labeling function $r :
\delta \rightarrow \{-W,\dots, W\}$, which assigns values between $-W$ and $W$ to edges. For a play $\pi =
e_0 e_1 e_2 \dots \in \delta^\omega, \Val(\overline{\pi}) = \lim \sup_{n\rightarrow\infty} \frac{1}{n+1} \sum_{i=0}^{n} r(e_i)$.
\fi





